FADE: Towards Fairness-aware Generation for Domain Generalization via Classifier-Guided Score-based Diffusion Models

Fairness-aware domain generalization (FairDG) has emerged as a critical challenge for deploying trustworthy AI systems, particularly in scenarios involving distribution shifts. Traditional methods for addressing fairness have failed in domain generalization due to their lack of consideration for distribution shifts. Although disentanglement has been used to tackle FairDG, it is limited by its strong assumptions. To overcome these limitations, we propose Fairness-aware Classifier-Guided Score-based Diffusion Models (FADE) as a novel approach to effectively address the FairDG issue. Specifically, we first pre-train a score-based diffusion model (SDM) and two classifiers to equip the model with strong generalization capabilities across different domains. Then, we guide the SDM using these pre-trained classifiers to effectively eliminate sensitive information from the generated data. Finally, the generated fair data is used to train downstream classifiers, ensuring robust performance under new data distributions. Extensive experiments on three real-world datasets demonstrate that FADE not only enhances fairness but also improves accuracy in the presence of distribution shifts. Additionally, FADE outperforms existing methods in achieving the best accuracy-fairness trade-offs.

==> abstract.tex <==
Fairness-aware domain generalization (FairDG) has emerged as a critical challenge for deploying trustworthy AI systems, particularly in scenarios involving distribution shifts. Traditional methods for addressing fairness have failed in domain generalization due to their lack of consideration for distribution shifts. Although disentanglement has been used to tackle FairDG, it is limited by its strong assumptions. To overcome these limitations, we propose Fairness-aware Classifier-Guided Score-based Diffusion Models (\sysname{}) as a novel approach to effectively address the FairDG issue. Specifically, we first pre-train a score-based diffusion model (SDM) and two classifiers to equip the model with strong generalization capabilities across different domains. Then, we guide the SDM using these pre-trained classifiers to effectively eliminate sensitive information from the generated data. Finally, the generated fair data is used to train downstream classifiers, ensuring robust performance under new data distributions. Extensive experiments on three real-world datasets demonstrate that \sysname{} not only enhances fairness but also improves accuracy in the presence of distribution shifts. Additionally, \sysname{} outperforms existing methods in achieving the best accuracy-fairness trade-offs.

==> introduction.tex <==
% % Graph structures, which represent entities and their relationships, have garnered widespread attention and application in real-world scenarios. Many graphs feature nodes associated with textual attributes, commonly referred to as text-attributed graphs. Examples include citation networks, social networks, e-commerce transaction networks, and hyperlink networks, all of which can be modeled as text-attributed graphs\cite{TAGbenchmark}. Current approaches\cite{TAGgraphformers,Tagexplanations} to learning from text-attributed graphs predominantly follow a two-step paradigm: first, extracting textual embeddings\cite{bert,roberta} and then applying Graph Neural Networks (GNN) \cite{GCN,GAT,Graphsage}, for message passing. These methods have achieved notable success. However, most traditional approaches rely on the assumption that the distribution of training and test data is consistent. When faced with out-of-distribution (OOD) data, such methods often misclassify OOD nodes as belonging to existing categories, leading to incorrect labels and reducing the model’s robustness and reliability. Consequently, detecting OOD anomalies while maintaining effective graph learning has become a critical challenge in this field.

% % This paper focuses on OOD detection at the node level in text-attributed graphs, where the goal is to ensure accurate node classification while identifying OOD nodes. Unlike OOD detection in vision\cite{cvoodsurvey} and text\cite{nlpoodsurvey} domains, where OOD samples are independent and identically distributed (i.i.d.), OOD detection in graph data is significantly more challenging due to the non-Euclidean nature of graph data and the interdependence of the data. Existing methods for graph-based OOD detection\cite{graphoodsurvey} are generally categorized into two main approaches: propagation-based methods and classification-based methods. The core motivation of propagation-based methods\cite{gpn,oodgat,ossnc} is to leverage the message-passing paradigm of GNNs to propagate existing uncertainty estimates, while classification-based\cite{msp,odin,graphsafe} methods focus on designing post hoc OOD score metrics for OOD detection. However, current methods often neglect the textual attributes and rely on shallow models (e.g., bag-of-words) for processing text features. This approach may miss crucial information embedded in the text attributes. Furthermore, existing models mainly depend on designing complex propagation mechanisms and uncertainty quantification metrics without fully considering the interplay between textual features and node connectivity. With the rapid development of large language models (LLM)\cite{glbench}, which possess extensive contextual knowledge and semantic understanding capabilities, textual attribute information can now be more fully captured and utilized. This enables us to approach the OOD detection problem from a novel perspective, leveraging LLM to better address the limitations of existing methods.

% % To tackle OOD detection in text-attributed graphs, we propose a novel LLM-enhanced contrastive learning-based method, named \textbf{LLM-Enhanced Energy Contrastive Learning for Out-of-Distribution Detection in Text-Attributed Graphs}. Our method consists of two main stages: (1) LLM-based sample generation and (2) energy-based contrastive learning. In the first stage, we construct empty pseudo-OOD nodes through random edge initialization. Then, utilizing the powerful textual understanding and generation capabilities of LLMs, we generate OOD samples that are related to the connected IND nodes through chain-of-thought (COT) prompts, producing high-quality pseudo-data with dependency relationships. In the second stage, we train the model using Linked IND-OOD Pairs and Triplet Contrastive Pairs, relying on an energy-based objective function to achieve precise OOD detection.

% % Our contributions are as follows:
% % \begin{itemize}[leftmargin=*]
% % \item We introduce a novel method for generating OOD samples in text-attributed graphs using large language models, resulting in high-quality OOD node textual attributes with dependency relationships.
% % \item We design a novel energy-based contrastive learning algorithm for OOD detection, enabling multi-dimensional sample pairs to effectively capture the differences between IND and OOD samples.
% % \item We demonstrate that our proposed model outperforms state-of-the-art baseline models on six benchmark datasets, while maintaining strong node classification performance.
% % \end{itemize}


% Graph structures, which represent entities and their relationships, have gained significant attention and application across various real-world scenarios. Many graphs, such as citation networks, social networks, e-commerce transaction networks, and hyperlink networks, feature nodes with textual attributes, commonly referred to as text-attributed graphs \cite{TAGbenchmark}. Current approaches to learning from text-attributed graphs \cite{TAGgraphformers,Tagexplanations} typically follow a two-step process: first, extracting textual embeddings \cite{bert,roberta,minilm}, followed by the application of Graph Neural Networks (GNN) \cite{GCN,GAT,Graphsage} for message passing. While these methods have achieved notable success, they are based on the assumption that the distribution of training and test data is consistent. When exposed to OOD data, these methods often misclassify OOD nodes as part of existing categories, leading to incorrect labels and undermining model robustness and reliability. Thus, detecting OOD anomalies while ensuring effective graph learning has become a critical challenge.

% This paper addresses node-level OOD detection in text-attributed graphs, focusing on accurate node classification while identifying OOD nodes. Unlike OOD detection in vision \cite{cvoodsurvey} and text \cite{nlpoodsurvey} domains, where OOD samples are assumed to be independent and identically distributed (i.i.d.), OOD detection in graph data is significantly more complex due to the non-Euclidean nature of graphs and the interdependence of their data. Existing methods for graph-based OOD detection \cite{graphoodsurvey} are generally categorized into propagation-based and classification-based approaches. Propagation-based methods \cite{gpn,oodgat,ossnc} leverage the message-passing paradigm of GNNs to propagate uncertainty estimates, while classification-based methods \cite{msp,odin,graphsafe} design post hoc OOD score metrics for detection. However, most current approaches overlook textual attributes and rely on shallow models (e.g., bag-of-words) for text processing, which may fail to capture crucial information embedded in the text. Furthermore, existing models often focus on complex propagation mechanisms and uncertainty quantification without adequately addressing the interaction between textual features and node connectivity. With the rapid advancement of large language models (LLMs) \cite{glbench}, which offer extensive contextual knowledge and semantic understanding, textual attribute information can now be more effectively captured and leveraged, offering a novel approach to OOD detection.\cite{cv_envisioning,nlpcontrastive,llmoodsurvey}

% To address OOD detection in text-attributed graphs, we propose a novel LLM-enhanced contrastive learning method, called \textbf{LLM-Enhanced Energy Contrastive Learning for Out-of-Distribution Detection in Text-Attributed Graphs}. Our method consists of two key stages: (1) LLM-based sample generation and (2) energy-based contrastive learning. In the first stage, we generate pseudo-OOD nodes by randomly initializing edges. Using the textual understanding and generation capabilities of LLMs, we create OOD samples related to connected IND nodes through chain-of-thought (COT) prompts, producing high-quality pseudo-data with dependency relationships. In the second stage, we train the model using Linked IND-OOD Pairs and Triplet Contrastive Pairs, applying an energy-based objective function to achieve precise OOD detection.

% Our contributions are as follows: \begin{itemize}[leftmargin=*] \item We propose a novel method for generating OOD samples in text-attributed graphs using large language models, resulting in high-quality OOD node textual attributes with dependency relationships. \item We design an energy-based contrastive learning algorithm for OOD detection, enabling multi-dimensional sample pairs to effectively capture the distinctions between IND and OOD samples. \item We demonstrate that our model outperforms state-of-the-art baselines on six benchmark datasets while maintaining strong node classification performance. \end{itemize}


Text-attributed graphs, which are a type of graph structure where nodes are associated with textual attributes, have gained significant attention due to their wide applicability in real-world scenarios, such as citation networks, social networks, e-commerce transaction networks, and hyperlink networks \cite{TAGbenchmark}. Current approaches to learning from text-attributed graphs \cite{TAGgraphformers,Tagexplanations} typically follow a two-step process: first, extracting textual embeddings \cite{bert,roberta,minilm}, and then applying Graph Neural Networks (GNNs) \cite{GCN,GAT,Graphsage} for message passing. While these methods have achieved notable success, they rely on the assumption that the distribution of training and test data is consistent. In the presence of out-of-distribution (OOD) data, these methods often misclassify OOD nodes as part of existing categories, undermining the model’s robustness and reliability. Thus, detecting OOD anomalies while ensuring effective graph learning has become a critical challenge.

We address the problem of node-level OOD detection in text-attributed graphs, with a focus on achieving accurate node classification while effectively identifying OOD nodes. Unlike OOD detection in vision \cite{cvoodsurvey} and language \cite{nlpoodsurvey}, where OOD samples are assumed to be independent and identically distributed (i.i.d.), OOD detection in graph data is significantly more complex due to the non-Euclidean nature of graphs and the interdependence of their data. Existing methods for graph OOD detection \cite{graphoodsurvey} can be categorized into propagation-based and classification-based approaches. Propagation-based methods \cite{gpn,oodgat,ossnc} leverage the message-passing paradigm of GNNs to propagate uncertainty estimates, while classification-based methods \cite{msp,odin,graphsafe} design OOD score metrics for detection. However, most current approaches overlook textual attributes and rely on shallow models, such as bag-of-words, which may fail to capture the rich semantic information embedded in the text. Furthermore, these models often focus on complex propagation mechanisms and uncertainty quantification, while neglecting the critical interplay between textual features and node connectivity. With the rapid advancement of large language models (LLMs) \cite{glbench}, which provide extensive contextual knowledge and semantic understanding, textual attribute information can now be more effectively captured and leveraged for OOD detection \cite{cv_envisioning,nlpcontrastive,llmoodsurvey}.

To address OOD detection in text-attributed graphs, we propose a novel LLM-enhanced contrastive learning method, named \textbf{LECT}. Our method consists of two key stages: (1) LLM-based sample generation and (2) energy-based contrastive learning. In the first stage, we generate pseudo-OOD nodes by randomly initializing edges. Using the textual understanding and generation capabilities of LLMs, we create OOD samples related to connected IND nodes through chain-of-thought (COT) prompts, producing high-quality pseudo-data with meaningful dependency relationships. In the second stage, we train the model using Linked IND-OOD Pairs and Triplet Contrastive Pairs, applying an energy-based objective function to effectively distinguish between IND and OOD samples. Our contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item We propose a novel method for generating high-quality OOD node textual attributes using LLMs, ensuring dependency relationships with connected IND nodes.
    \item We design an energy-based contrastive learning algorithm for OOD detection, which enables multi-dimensional sample pairs to effectively capture distinctions between IND and OOD samples.
    \item We demonstrate that our model outperforms state-of-the-art baselines on six benchmark datasets while maintaining strong node classification performance.
\end{itemize}

